A Discussion of Thin Client Technology for Computer Labs

Computer literacy is not negotiable for any professional in an increasingly computerised environment. Educational institutions should be equipped to provide this new basic training for modern life. Accordingly, computer labs are an essential medium for education in almost any field. Computer labs are one of the most popular IT infrastructures for technical training in primary and secondary schools, universities and other educational institutions all over the world. Unfortunately, a computer lab is expensive, in terms of both initial purchase and annual maintenance costs, and especially when we want to run the latest software. Hence, research efforts addressing computer lab efficiency, performance or cost reduction would have a worldwide repercussion. In response to this concern, this paper presents a survey on thin client technology for computer labs in educational environments. Besides setting out the advantages and drawbacks of this technology, we aim to refute false prejudices against thin clients, identifying a set of educational scenarios where thin clients are a better choice and others requiring traditional solutions.

==> Makefile <==
all : ictel2010.pdf

ictel2010.pdf : ictel2010.dvi
	dvipdf $^

ictel2010.dvi : ictel2010.tex ictel2010.aux \
	authors.tex abstract.tex keywords.tex title.tex \
	introduction.tex background.tex strengths.tex survey.tex
	latex $<
	latex $<

ictel2010.aux : ictel2010.tex
	latex $<
	bibtex ictel2010


==> abstract.tex <==
\fontsize{9}{11}\selectfont Computer literacy is not negotiable for any professional in an increasingly computerised environment. Educational institutions should be equipped to provide this new basic training for modern life. Accordingly, computer labs are an essential medium for education in almost any field. Computer labs are one of the most popular IT infrastructures for technical training in primary and secondary schools, universities and other educational institutions all over the world. Unfortunately, a computer lab is expensive, in terms of both initial purchase and annual maintenance costs, and especially when we want to run the latest software. Hence, research efforts addressing computer lab efficiency, performance or cost reduction would have a worldwide repercussion. In response to this concern, this paper presents a survey on thin client technology for computer labs in educational environments. Besides setting out the advantages and drawbacks of this technology, we aim to refute false prejudices against thin clients, identifying a set of educational scenarios where thin clients are a better choice and others requiring traditional solutions.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Jes\'us Mart\'inez-Mateo, Susana Munoz-Hernandez, David P\'erez-Rey\\
  \fontsize{9}{11}\selectfont
  \textit{Facultad de Inform\'atica, Universidad Polit\'ecnica de Madrid, Campus de Montegancedo, Spain}\\
  \fontsize{9}{11}\selectfont
  \textit{jmartinez@fi.upm.es, susana@fi.upm.es, dperezdelrey@fi.upm.es}\\[12pt]
  %
  %\fontsize{11}{13}\selectfont
  %Third Author Name\\
  %\fontsize{9}{11}\selectfont
  %\textit{Department of Computing, Main University, MySecondTown, MyCountry}\\
  %\fontsize{9}{11}\selectfont
  %\textit{t\_author@xy.mu.edu}\\[12pt]
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont thin client, e-learning, computer lab.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{A Discussion of Thin Client Technology for Computer Labs}
}

